On the Probability of Network States with Gaussian Connectivity Functions

In this paper, we consider the connectivity of a random network of N mobile devices in three dimensions (3D), where the location of each device or node has a Gaussian distribution in each dimension. For each pair of nodes, the probability of connectivity is related to the nodes' separation by a Gaussian connectivity function. The fundamental analytical tool for studying such systems is the probability of a given network state, derived and expressed in terms of its graph Laplacian. Leveraging this result, we obtain results for the connectivity of small networks, the probability of a complete network (where all nodes are connected to all other nodes), and the probability of an isolated node, which gives an approximation to the connectivity probability of larger networks. The general results are then simplified for special cases and limiting scenarios.

==> N1.tikz.tex <==
\begin{circuitikz}
\tikzstyle{every node}=[font=\Huge]
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (0.75,0) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (11.25,0) circle (0.5cm);
\node [font=\LARGE] at (0.75,0) {$n_1$};
\node [font=\LARGE] at (11.25,0) {$n_4$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (6,1.5) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (6,-1.5) circle (0.5cm);
\node [font=\LARGE] at (6,1.5) {$n_2$};
\node [font=\LARGE] at (6,-1.5) {$n_3$};
\draw [line width=1.5pt](1.25,0) to[short] (5.5,1.5);
\draw [line width=1.5pt](1.25,0) to[short] (5.5,-1.5);
\draw [line width=1.5pt](6.5,-1.5) to[short] (10.75,0);
\draw [line width=1.5pt](6,1) to[short] (6,-1);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}](6.5,1) to (6.5,-1);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}] (1.25,-0.5) to (5.5,-2);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}] (1.25,0.5) to (5.5,2);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}] (6.75,-2) to (10.75,-0.5);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}] (6.75,2) to (10.75,0.5);
\draw [<->, >=Stealth,line width=1.5pt,color={rgb,255:red,60; green,140; blue,226}] (0.75,-2.5) to (11.25,-2.5);
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (6,-3) {$r_{14}$};
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (7.15,0) {$r_{23}$};
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (3.25,-1.6) {$r_{13}$};
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (9,-1.6) {$r_{34}$};
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (3.25,1.75) {$r_{12}$};
\node [font=\LARGE,color={rgb,255:red,60; green,140; blue,226}] at (9,1.75) {$r_{24}$};
\end{circuitikz}

==> threenode.tikz.tex <==
\begin{circuitikz}
\tikzstyle{every node}=[font=\LARGE]
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (0,0) circle (0.5cm);
\node [font=\LARGE] at (0,0) {$n_1$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (3,2) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (6,0) circle (0.5cm);
\node [font=\LARGE] at (3,2) {$n_2$};
\node [font=\LARGE] at (6,0) {$n_3$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (8.5,0) circle (0.5cm);
\node [font=\LARGE] at (8.5,0) {$n_1$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (11.5,2) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (14.5,0) circle (0.5cm);
\node [font=\LARGE] at (11.5,2) {$n_2$};
\node [font=\LARGE] at (14.5,0) {$n_3$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (0,-4) circle (0.5cm);
\node [font=\LARGE] at (0,-4) {$n_1$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (3,-2) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (6,-4) circle (0.5cm);
\node [font=\LARGE] at (3,-2) {$n_2$};
\node [font=\LARGE] at (6,-4) {$n_3$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (8.5,-4) circle (0.5cm);
\node [font=\LARGE] at (8.5,-4) {$n_1$};
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (11.5,-2) circle (0.5cm);
\draw [ fill={rgb,255:red,254; green,255; blue,255} , line width=1.5pt ] (14.5,-4) circle (0.5cm);
\node [font=\LARGE] at (11.5,-2) {$n_2$};
\node [font=\LARGE] at (14.5,-4) {$n_3$};
\draw [line width=1.5pt, short] (0.5,0) -- (5.5,0);
\draw [line width=1.5pt, short] (0,0.5) -- (2.5,2);
\draw [short] (1.25,1) -- (1.25,1);
\draw [line width=1.5pt, short] (3.5,2) -- (6,0.5);
\draw [line width=1.5pt, short] (8.5,0.5) -- (11,2);
\draw [line width=1.5pt, short] (12,2) -- (14.5,0.5);
\draw [line width=1.5pt, short] (0,-3.5) -- (2.5,-2);
\draw [line width=1.5pt, short] (0.5,-4) -- (5.5,-4);
\draw [line width=1.5pt, short] (9,-4) -- (14,-4);
\draw [line width=1.5pt, short] (12,-2) -- (14.5,-3.5);
\node [font=\LARGE] at (3,-0.75) {a. $G_1$};
\node [font=\LARGE] at (11.75,-0.75) {b. $G_2$};
\node [font=\LARGE] at (3,-4.75) {c. $G_3$};
\node [font=\LARGE] at (11.75,-4.75) {d. $G_4$};
\end{circuitikz}
